Decentralized Quadratically Approximated Alternating Direction Method of Multipliers

This paper considers an optimization problem that components of the objective function are available at different nodes of a network and nodes are allowed to only exchange information with their neighbors. The decentralized alternating method of multipliers (DADMM) is a well-established iterative method for solving this category of problems; however, implementation of DADMM requires solving an optimization subproblem at each iteration for each node. This procedure is often computationally costly for the nodes. We introduce a decentralized quadratic approximation of ADMM (DQM) that reduces computational complexity of DADMM by minimizing a quadratic approximation of the objective function. Notwithstanding that DQM successively minimizes approximations of the cost, it converges to the optimal arguments at a linear rate which is identical to the convergence rate of DADMM. Further, we show that as time passes the coefficient of linear convergence for DQM approaches the one for DADMM. Numerical results demonstrate the effectiveness of DQM.

==> Conclusions.tex <==
%!TEX root = root.tex

\section{Conclusions}

\newpage

==> Convergence.tex <==
%!TEX root = root.tex

\section{Convergence Analysis}\label{sec:convergence_analysis}




In this section we show that as time progresses the sequence of objective function $F(\bby_t)$ defined in \eqref{centralized_opt_problem} approaches the optimal objective function value $F(\bby^{*})$. In proving this claim we make the following assumptions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%     A   S   S   U   M   P   T   I   O   N      %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{assumption}\label{ass_weight_bounds} There exists constants $0\leq\delta<\Delta<1$ that lower and upper bound the diagonal weights for all $i$, 
%
\begin{equation}\label{bounds_for_local_weights}
   0\leq \delta  \leq w_{ii} \leq \Delta <1  \qquad  i=1,\ldots,n .
\end{equation}\end{assumption}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%     A   S   S   U   M   P   T   I   O   N      %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{assumption}\label{convexity_assumption} 
The local objective functions $f_i(\bbx)$ are twice differentiable and strongly convex with parameter $m>0$.
\end{assumption}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A S S U M P T I O N S   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{assumption}\label{Lipschitz_assumption} The local objective function Hessians $\nabla^2 f_i(\bbx)$ are Lipschitz continuous with parameter $L$ with respect to Euclidian norm  for all $\bbx, \hbx \in \reals^p$, i.e.
%
\begin{equation}
   \| \nabla^2 f_i(\bbx)-\nabla^2 f_i(\hbx) \| \ \leq\  L\ \| \bbx- \hbx \|.
\end{equation}
\end{assumption}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  M  A  I  N      M  A  T  T  E  R  %%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The upper bound $\Delta$ for the local wights in Assumption \ref{ass_weight_bounds} is imposed by the connectivity assumption. Connectivity of network guarantees that each node has at least one neighbor and this observation in association with the condition that the sum of weight for each node is 1, i.e.$\sum_{j}w_{ij}=1$, implies that the local weights are strictly smaller than 1. Therefore, there exits a positive constant $\Delta <1$ as an upper bound for local weights $w_{ii}$. The existence of lower bound $0 \leq \delta$ is implied by the condition that all the weights $w_{ij}$ are non-negative.

Assumption \ref{convexity_assumption} implies that all the eigenvalues of local Hessians are larger than $m$, i.e., $m\bbI\preceq \nabla^2 f_{i}(\bbx)$ for all $\bbx \in \reals^p$ and $i\in\{1,\dots,n\}$. Strong convexity implies that the sublevel sets contained in $\bbx \in \reals^p$ are bounded and as a result the maximum eigenvalue of $\nabla^2 f_{i}(\bbx)$ is bounded above. Hence, eigenvalues of local Hessian matrices $\nabla^2 f_{i}(\bbx)$ are bounded with positive constants $0<m\leq M<\infty$, i.e.
%
\begin{equation}\label{local_hessian_eigenvlaue_bounds}
m\bbI\preceq \nabla^2 f_i(\bbx)\preceq M\bbI,
\end{equation}
%%
for all $\bbx \in \reals^p$ and $i\in\{1,\dots,n\}$. The strong convexity assumption for the local objective functions $f_{i}(\bbx)$ stated in Assumption \ref{convexity_assumption} is customary in convergence proofs of Newton-based methods, since the Hessian of objective function should be invertible to establish Newton method \cite{boyd}. 




The restriction imposed by Assumption \ref{Lipschitz_assumption} is typical of second order methods in proving super-linear convergence \cite{boyd,ZarghamEtal14}. Assumption \ref{Lipschitz_assumption} guarantees that the Hessian matrices of objective functions $F(\bby)$ are also Lipschitz continuous as we show in the following lemma.


 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% L   E   M   M   A %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{Hessian_Lipschitz_countinous}
Consider the definition of objective function $F(\bby)$ in \eqref{centralized_opt_problem}. If Assumption \ref{Lipschitz_assumption} holds then the objective function Hessian $\bbH(\bby) =: \nabla^2F(\bby)$ is Lipschitz continuous with parameter $\alpha L$, i.e.
%
\begin{equation}\label{H_Lipschitz_claim}
\left\|\bbH(\bby)-\bbH(\hby)\right\| \leq \alpha L \| \bby-\hby\| .
\end{equation}
%
for all $\bby,\hby\in \reals^{np}$.
\end{lemma}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% P   R   O   O   F %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{myproof}
See Appendix \ref{app_Hessian_Lipschitz}.
\end{myproof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% M A I N    M A T T E R %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Lemma \ref{Hessian_Lipschitz_countinous} states that the penalty objective function introduced in  \eqref{centralized_opt_problem} has the property that the Hessians are Lipschitz continuous, while the Lipschitz constant is a function of penalty coefficient $1/\alpha$. This observation implies as we increase the penalty coefficient $1/\alpha$ or equivalently decrease $\alpha$, the objective function $F(\bby)$ approaches a quadratic objective function. To verify this result consider the case that $\alpha=0$. In this case the objective function can be written as $F(\bby)=(1/2)\bby^T(\bbI-\bbZ)\bby$ which is a quadratic function.

To prove convergence properties of NN method the bounds for the eigenvalues of block diagonal matrix $\bbD_t$, positive semi-definiteness $\bbB$, and the Hessian $\bbH_t$ are necessary. In the following proposition we characterize bounds for the eigenvalues of these matrices using the conditions imposed by Assumptions \ref{ass_weight_bounds} and \ref{convexity_assumption}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  P  R  O  P  O  S  I  T  I  O  N  %%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}\label{eigenvalue_bounds}
Consider the definitions of matrices $\bbH_t$, $\bbD_t$, and $\bbB$ in \eqref{Hessian}, \eqref{diagonal_matrix}, and \eqref{non_diagona_matrix}, respectively. If Assumptions \ref{ass_weight_bounds} and \ref{convexity_assumption} hold true, the eigenvalues of matrices $\bbH_t$, $\bbD_t$, and $\bbB$ are uniformly bounded as 
%
\begin{align}
 \alpha m \bbI\ \preceq \ & {\bbH_t} \ \preceq \ (2(1-\delta) + \alpha M)\bbI ,\\
 (2(1-\Delta)+\alpha m) \bbI\ \preceq\ & {\bbD_t}\ \preceq\ (2(1-\delta)+\alpha M)\bbI ,\\
 \bb0\ \preceq\ & \ {\bbB}\ \preceq\ 2 (1-\delta) \bbI.
\end{align}
%
\end{proposition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  P  R  O  O  F  %%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{myproof} 
See Appendix \ref{app_eigenvalue_bounds}.  
\end{myproof}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  M  A  I  N      M  A  T  T  E  R  %%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Proposition \ref{eigenvalue_bounds} states that Hessian matrix $\bbH_t$ and block diagonal matrix $\bbD_t$ are positive definite, while matrix $\bbB$ is positive semidefinite. For the expansion in \eqref{exact_Hessian_inverse} to be valid the eigenvalues of matrix $\bbD_t^{-{1}/{2}}\bbB\bbD_t^{-{1}/{2}}$ must be nonnegative and strictly smaller than $1$. The following proposition states that this is true for all $t$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  P  R  O  P  O  S  I  T  I  O  N  %%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}\label{symmetric_term_bounds11}
Consider the definitions of matrices $\bbD_t$ in \eqref{diagonal_matrix} and $\bbB$ in \eqref{non_diagona_matrix}. If Assumptions \ref{ass_weight_bounds} and \ref{convexity_assumption} hold true, the matrix $\bbD_t^{-{1}/{2}}  \bbB   \bbD_t^{-{1}/{2}}$ is positive semidefinite and the eigenvalues are bounded above by a constant $\rho<1$
%
\begin{equation}\label{important_claim}
    \bb0\  \preceq \  \bbD_t^{-{1}/{2}}  \bbB   \bbD_t^{-{1}/{2}} \ \preceq\ \rho\bbI ,
\end{equation}
%%
where $\rho:= 2(1-\delta)/(2(1-\delta)+{\alpha m} )$.
%
\end{proposition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  P  R  O  O  F  %%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{myproof}
See Appendix \ref{app_eigenvalue_of_DBD}.
\end{myproof} 

The bounds for the eigenvalues of matrix $\bbD_t^{-{1}/{2}}  \bbB   \bbD_t^{-{1}/{2}}$ in \eqref{important_claim} guarantee convergence of Taylor series in \eqref{exact_Hessian_inverse}. As mentioned in Section \ref{subsec_nn}, NN-$K$ truncates the first $K$ summands of Hessian inverse Taylor series in \eqref{exact_Hessian_inverse} to approximate the Hessian inverse of objective function in optimization problem \eqref{centralized_opt_problem}. To evaluate the performance of NN-$K$ method we study the error of Hessian inverse approximation by defining \textit{error matrix} $\bbE_t\in\reals^{np\times np}$ as  
%%
\begin{equation}\label{error_matrix}
\bbE_t:= \bbI- {\hbH_{t}^{(K)^{-{1}/{2}}}} \bbH_t  {\hbH_{t}^{(K)^{-{1}/{2}}}}.
\end{equation}
%%
Error matrix $\bbE_t$ measures closeness of the Hessian inverse approximation matrix $\hbH_{t}^{-1}$ and the exact Hessian inverse $\bbH^{-1}_t$ at time $t$. Based on the definition of error matrix $\bbE_t$, as the Hessian inverse approximation $\hbH_{t}^{-1}$ approaches to the exact Hessian inverse $\bbH_t^{-1}$ the error matrix $\bbE_t$ approaches zero matrix $\bb0$. In the following proposition we study the error of Hessian inverse approximation by studying bounds for the eigenvalues of error matrix $\bbE_t$. Further, we show that by increasing the level of approximation $K$, the error of Hessian inverse approximation for NN-$K$ decreases.










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  P R O P O S I T I O N %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proposition}\label{error_matrix_proposition}
Consider the NN-$K$ method as introduced in \eqref{diagonal_matrix}-\eqref{update_formula_NN} and the definition of error matrix $\bbE_t$ as in \eqref{error_matrix}. Further, recall the definition of constant $\rho<1$ in Proposition \ref{symmetric_term_bounds11} that $\rho :=2(1-\delta)/(\alpha+2(1-\delta))$. Then, the error matrix $\bbE_t$ is positive semi-definite and all the eigenvalues are upper bounded as
%
\begin{equation}\label{bound_for_error}
    \bb0\  \preceq\ \bbE_t\ \preceq\ \rho^{K+1}\bbI.
\end{equation}
%
\end{proposition}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%  P   R   O   O   F  %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{myproof}
See Appendix \ref{app_error_matrix}.
\end{myproof}
 %

Proposition \ref{error_matrix_proposition} asserts that the error in the approximation of the Hessian inverse -- thereby on the approximation of the Newton step -- is bounded by $\rho^{K+1}$. This result corroborates the intuition that the larger $K$ is, the closer that $\bbd_{i,t}^{(K)}$ approximates the Newton step. This closer approximation comes at the cost of increasing the communication cost of each descent iteration. The decrease of this error being proportional to $\rho^{K+1}$ hints that using $K=1$ or $K=2$ should provide good enough approximations. This is true in practice -- see Section \ref{sec:simulations}. To decrease $\rho$ we can increase $\delta$ or $\alpha$. Increasing $\delta$ calls for assigning substantial weight to $w_{ii}$. Increasing $\alpha$ comes at the cost of moving the solution of \eqref{centralized_opt_problem} away from the solution of \eqref{original_optimization_new_notation} and its equivalent \eqref{original_optimization_problem1}.




The assumption that the eigenvalues of objective function Hessian $\bbH_t$ are bounded has a significant role in the convergence analysis of Newton's method \cite{boyd}. The lower bound for the eigenvalues of Hessian guarantees that the matrix is nonsingular and the upper bound implies that the minimum eigenvalue of Hessian inverse $\bbH^{-1}$ is strictly larger than zero which implies decrement in each step of Newton method. The same bounds for the eigenvalues of the Network Newton approximate Hessian inverse $ {\hbH_{t}^{(K)^{-1}}}$ are required. These bounds are studied in the following lemma.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% L   E   M   M   A %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{Hessian_inverse_eigenvalue_bounds_lemma}
Consider the NN-$K$ method as defined in \eqref{diagonal_matrix}-\eqref{update_formula_NN}. If Assumptions \ref{ass_weight_bounds} and \ref{convexity_assumption} hold true, the eigenvalues of approximate Hessian inverse $\hbH_t^{(K)^{-1}}$ are bounded as
%%
\begin{equation}\label{bounded_Hessian_inverse}
\lambda \bbI\ \preceq\  \hbH_t^{(K)^{-1}}\  \preceq\   \Lambda \bbI,
\end{equation} 
%%
where constants $\lambda$ and $\Lambda$ are defined as
\begin{equation}\label{definition_of_lambdas}
\!\!\! \lambda\!:=\! \frac{1}{2(1-\delta)+\alpha M } \ \text{ and} 
\ \ \Lambda\! :=\! {\frac{1-\rho^{K+1}}{(1-\rho)(2(1-\Delta)+\alpha m )}}.
\end{equation}
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% P   R   O   O   F %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{myproof}
See Appendix \ref{app_eigenvalues_of_Hessian__inverse_approximation}.
\end{myproof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% M A I N    M A T T E R %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

According to the result of Lemma \ref{Hessian_inverse_eigenvalue_bounds_lemma} the NN-$K$ approximate Hessian inverse $\hbH_t^{(K)^{-1}}$ is strictly positive definite and all the eigenvalues bounded above. Note that even for the case that $K\to \infty$, still the lower and upper bounds in \eqref{definition_of_lambdas} are finite. Considering the bounds for the eigenvalues of the approximate Hessian inverse $\hbH_t^{(K)^{-1}}$ and the fact that $-\bbg_t$ is a descent direction as it has been shown for DGD, the approximate Newton step $-\hbH_t^{(K)^{-1}}\bbg_t$ enforces convergence for the iterate $\bby_t$ as well as for the objective function sequence $F(\bby_{t})$. In the following theorem we show that if stepsize $\epsilon$ is properly chosen, then the sequence of objective function $F(\bby_t)$ converges at least linearly to the optimal objective function $F(\bby^*)$.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   T   H   E   O   R   E   M   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{thm}\label{linear_convergence}
Consider the NN-$K$ method as defined in \eqref{diagonal_matrix}-\eqref{update_formula_NN} and the objective function $F(\bby)$ as introduced in \eqref{centralized_opt_problem}. If the stepsize $\epsilon$ is chosen as 
%
\begin{equation}\label{step_size_condition}
\epsilon = \min  \left\{ 1\ , \left[{\frac{3m\lambda^{\frac{5}{2}}}{ L\Lambda^{3}{(F(\bby_{0})-F(\bby^{*})) }^{\frac{1}{2}} } }  \right]^{\frac{1}{2}} \right\} 
\end{equation}
%
and Assumptions \ref{ass_weight_bounds}, \ref{convexity_assumption}, and \ref{Lipschitz_assumption} hold true, the sequence $F(\bby_{t})$ converges to the optimal argument $F(\bby^{*})$ at least linearly with constant $1-\zeta$. I.e.,
%
%
\begin{equation}\label{linear_convegrence_claim}
F(\bby_{t}) -F(\bby^*) \leq (1-\zeta)^t  {\left(F(\bby_{0}) -F(\bby^*) \right)},
\end{equation}
%
where the constant $0<\zeta<1$ is explicitly given by
%
\begin{equation}\label{beta_0_defintion}
\zeta :=    {(2-\eps) \epsilon\alpha m\lambda} - \frac{\alpha\epsilon^3  L\Lambda^{3}(F(\bby_{0})-F(\bby^{*}) )^{\frac{1}{2}}}{6\lambda^{\frac{3}{2}}} .
\end{equation}
%%
\end{thm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%  P    R    O     O      F   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{myproof}
See Appendix \ref{app_linear_convergecene_theorem}.
\end{myproof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  M A I N     M A T T E R     %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Theorem \ref{linear_convergence} shows that the objective function error sequence $F(\bby_t)-F(\bby^{*})$ asymptoticly converges to zero and that the rate of convergence is at least linear. Note that according to the definition of the convergence parameter $\zeta $ in Theorem \ref{linear_convergence} and the definitions of $\lambda$ and $\Lambda$ in \eqref{definition_of_lambdas}, increasing $\alpha$ leads to faster convergence. This observation verifies existence of a tradeoff between rate and accuracy of convergence. For large values of $\alpha $ the sequence generated by Network Newton converges faster to the optimal solution of \eqref{centralized_opt_problem}, while the accuracy of convergence is low since the parameter $\alpha$ is large. Smaller $\alpha $ implies smaller gap between the optimal solutions of \eqref{centralized_opt_problem} and \eqref{original_optimization_problem1}, but the convergence rate of NN-$K$ is slower.



\subsection{Rate of convergence}


Theorem \ref{linear_convergence} shows linear convergence of sequence generated by NN-$K$ method, however, this result is similar to the convergence properties of DGD. Given that NN-$K$ tries to approximate the Newton step, we expect to observe some form of superlinear convergence. To characterize convergence rate of NN-$K$ method, first we study the difference between this algorithm and the exact Newton's methods. The following lemma shows that convergence properties of the norm of weighted gradient $\|\bbD_{t-1}^{-{1}/{2}}\bbg_{t}\|$ in NN-$K$ are similar to the convergence of Newton method with constant step-size. The difference is the appearance of a term that corresponds to the error of the Hessian inverse approximation.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   L   E   M   M   A   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{lemma}\label{two_phase_convergence_lemma}
Consider the NN-$K$ method as defined in \eqref{diagonal_matrix}-\eqref{update_formula_NN}. If Assumptions \ref{ass_weight_bounds}, \ref{convexity_assumption}, and \ref{Lipschitz_assumption} hold true, then
%%%
%%
\begin{align}\label{convg_rate_lemma_claim}
\left\|\bbD_{t}^{-{1}/{2}}\bbg_{t+1}\right\|  & \!\leq \! 
	   \left(1-\eps+ \eps \rho^{K+1}\right) \!\!\left[1\! +\!  \Gamma_1 (1-\zeta)^{\frac{(t-1)}{4}} \right]\! \!\left\|\bbD_{t-1}^{-{1}/{2}}\bbg_{t}\right\| \nonumber \\	
	   & \qquad + \eps^2 \Gamma_2 \left\| \bbD_{t-1}^{-{1}/{2}}\bbg_{t}\right\|^2,
\end{align}
%%
where $\Gamma_1$ and $\Gamma_2$ are defined as 
%%
\begin{equation}\label{Gammas_definition}
    \Gamma_1 \!:=\! {\frac{(\alpha \eps L\Lambda)^{\frac{1}{2}}  (F(\bby_{0}) -F(\bby^*) )^{\frac{1}{4}}}{\lambda^{\frac{3}{4}}(2(1-\Delta)+\alpha m) }} 
	, \Gamma_2 \!:=\!	 \frac{ \alpha L\Lambda^2}{2\lambda {(2(1-\Delta)+\alpha m)}^{\frac{1}{2}}}.
\end{equation}
\end{lemma}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  P   R   O   O   F  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{myproof}
See Appendix \ref{App_two_phase_convergence_lemma}.
\end{myproof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  M  A   I   N      M   A   T   T   E   R  %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As per Lemma \ref{two_phase_convergence_lemma} the weighted gradient norm $\|\bbD_{t}^{-{1}/{2}}\bbg_{t+1}\|$ is upper bounded by terms that are linear and quadratic on the weighted norm $\|\bbD_{t-1}^{-{1}/{2}}\bbg_{t}\|$ associated with the previous iterate. This is akin to the gradient norm decrease of Newton's method with constant stepsize. Further note that for all except the first few iterations $\Gamma_1 (1-\zeta)^{(t-1)/4}\approx 0$. In that case the coefficient in the linear term reduces to $(1-\eps+ \eps \rho^{K+1})$ which is strictly smaller than 1, i.e. $(1-\eps+ \eps \rho^{K+1})<1$. Furthermore, by making $\eps=1$ the upper bound in \eqref{convg_rate_lemma_claim} becomes $\rho^{K+1}\| \bbD_{t-1}^{-\frac{1}{2}}\bbg_{t}\|+ \Gamma_2\| \bbD_{t-1}^{-\frac{1}{2}}\bbg_{t}\|^2$, implying that there must be intervals in which the quadratic term dominates and NN-$K$ exhibits quadratic convergence. We state this fact formally in the following theorem. 








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   T   H   E   O   R   E   M   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{thm}\label{quadratic_convergence_theorem}
Consider the NN-$K$ method as introduced in \eqref{diagonal_matrix}-\eqref{update_formula_NN} and define the sequence $\eta_{t} :=[(1-\eps+\eps\rho^{K+1})(1 +  \Gamma_1 (1-\zeta)^{{(t-1)}/{4}} ) ]$. Further, define $t_0$ as the first time that sequence $\eta_t$ is smaller than 1, i.e. $t_0:= \argmin_{t}\{ t \mid \eta_t<1\}$.
%%%
%\vspace{-1mm}
%\red{
%%%
%\begin{equation}\label{t0_definition}
%t_0= \argmin_{t} \left\{t\ \Big{| } \  \Big[1-\eps+ \eps \rho^{K+1} \Big] \left[1 +  \Gamma_1 (1-\zeta)^{\frac{t-1}{4}} \right]\!<1\! \right\}.\vspace{-1mm}
%\end{equation}
%%%
%}
If Assumptions  \ref{ass_weight_bounds}, \ref{convexity_assumption}, and \ref{Lipschitz_assumption} hold true, for all $t\geq t_0$ when the sequence $\|\bbD_{t-1}^{-1/2}\bbg_{t}\|$ satisfies 
%%
\begin{equation}\label{interval_condition}
	\frac{\sqrt{\eta_{t}}(1- \sqrt{\eta_t}) }{ \eps^2\Gamma_2} 
	\leq\left\|\bbD_{t-1}^{-1/2}\bbg_{t}\right\|
	< \frac{1- \sqrt{\eta_t}}{ \eps^2\Gamma_2}\ ,
\end{equation}
%%
the rate of convergence is quadratic in the sense that
%%
\begin{equation}\label{super_linear_claim_theorem}
{\left\|\bbD_{t}^{-1/2}\bbg_{t+1}\right\|} \leq \frac{\eps^2 \Gamma_2}{1-\sqrt{\eta_t}} {\left\|\bbD_{t-1}^{-1/2}\bbg_{t}\right\|}^{2}.
\end{equation}
%%
\end{thm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%     P   R   O   O   F     %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{myproof} Considering the definition of $\eta_{t}$ we can rewrite the result of Lemma \ref{two_phase_convergence_lemma} as
%%
\begin{equation}\label{safa_city}
\left\|\bbD_{t}^{-{1}/{2}}\bbg_{t+1}\right\|   \leq 
	\eta_t \left\|\bbD_{t-1}^{-{1}/{2}}\bbg_{t}\right\| + \eps^2 \Gamma_2 \left\| \bbD_{t-1}^{-{1}/{2}}\bbg_{t}\right\|^2.
\end{equation}
%%
we use this result to prove that the inequality in \eqref{super_linear_claim_theorem} holds true.
Considering the lower bound of interval that sequence ${\|\bbD_{t-1}^{-1/2}\bbg_{t}\|}$ is in as introduced in \eqref{interval_condition}, we can write
%%
\begin{equation}\label{yek_chi_begim_bere}
{\sqrt{\eta_{t}}}\ \leq\ \frac{\eps^2   \Gamma_2}{1- \sqrt{\eta_t}} \left\| \bbD_{t-1}^{-1/2}\bbg_{t}\right\|.
\end{equation}
%%
Multiplying both sides of \eqref{yek_chi_begim_bere} by $\sqrt{\eta_t}\| \bbD_{t-1}^{-1/2}\bbg_{t}\|$ implies that 
%%
\begin{equation}\label{yek_chi_begim_bere_2}
\eta_t \left\|\bbD_{t-1}^{-{1}/{2}}\bbg_{t}\right\|  
	\leq\frac{\sqrt{\eta_t}\eps^2   \Gamma_2}{1- \sqrt{\eta_t}}\left\| \bbD_{t-1}^{-1/2}\bbg_{t}\right\|^2.
\end{equation}
%%
Substituting $\eta_t\|\bbD_{t-1}^{-\frac{1}{2}}\bbg_{t}\|  $ in \eqref{safa_city} by the upper bound in \eqref{yek_chi_begim_bere_2} implies that 
%%
\begin{align}\label{super_linear_phase}
\left\|\bbD_{t}^{-{1}/{2}}\bbg_{t+1}\right\| 
  &\leq \frac{\sqrt{\eta_t}\eps^2   \Gamma_2}{1- \sqrt{\eta_t}} \left\| \bbD_{t-1}^{-1/2}\bbg_{t}\right\|^2
  + \eps^2 \Gamma_2 \left\| \bbD_{t-1}^{-{1}/{2}}\bbg_{t}\right\|^2	\nonumber \\
  &= \frac{\eps^2   \Gamma_2}{1- \sqrt{\eta_t}} \left\| \bbD_{t-1}^{-1/2}\bbg_{t}\right\|^2.
\end{align}
%%
To verify quadratic convergence, it is necessary to prove that  the sequence of weighted gradient $\| \bbD_{i-1}^{-1/2}\bbg_{i}\|$ is decreasing or equivalently
%%
\begin{equation}\label{less_than_1}
\frac{\eps^2   \Gamma_2}{1- \sqrt{\eta_t}} \left\| \bbD_{t-1}^{-1/2}\bbg_{t}\right\|< 1,
\end{equation}
%%
which this result follows by considering the upper bound of the interval in \eqref{interval_condition}.
\end{myproof}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% %      M A I  N     M A T T E  R       %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Theorem \ref{quadratic_convergence_theorem} shows that the sequence of weighted gradients $\|\bbD_{t-1}^{-1/2}\bbg_{t}\|$ generated by NN-$K$ decays quadratically in the specified interval. That interval is not empty, since for $t
\geq t_0$ we have $\sqrt{\eta_t}<1$. Note that outside of this interval linear convergence still holds as a result of Theorem \ref{linear_convergence}.

\red{
\begin{remark}
{For quadratic objective function where the Lipschitz constant is $L=0$, the optimal choice of stepsize for NN-$K$ is $\eps=1$ and constants for the linear and quadratic terms in \eqref{convg_rate_lemma_claim} are $\Gamma_1=\Gamma_2=0$. Hessian of objective function $\bbH_t$ and diagonal matrix $\bbD_{t}$ are constant which implies that we can rewrite \eqref{convg_rate_lemma_claim} as $\|\bbD^{-{1}/{2}}\bbg_{t+1}\| \leq \rho^{K+1}\|\bbD^{-{1}/{2}}\bbg_{t}\| $. Therefore, the sequence converges lineally with parameter $\rho^{K+1}$ which does not depend on the condition number of problem. Note that for the Newton method only one step of iteration is required for convergence.}
\end{remark}
}




==> Implementation.tex <==
%!TEX root = root.tex

\section{Network Newton Implementation} \label{sec:implement}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   L   G   O   R   I   T   H   M   %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{algorithm}[t]
\caption{Adaptive Network Newton-$K$ method at node $i$}\label{algo_ANN} 
\begin{algorithmic}[1] {
\REQUIRE  Initial iterate $\bbx_{i,0}$, initial penalty parameter $\alpha_0$ and initial sequence of bits $\bbs_i=[s_{i1};\dots;s_{in}]=[0;\dots;0].$
\FOR {$t=0,1,2,\ldots$}
   \STATE Exchange iterates $\bbx_{i,t}$ with neighbors $j\in \mathcal{N}_i$.
   \STATE Gradient:    
          %
          $\displaystyle{
          \bbg_{i,t}\! =\! (1-w_{ii})\bbx_{i,t} 
                       \!-\! \sum_{j\in \mathcal{N}_i} \! w_{ij} \bbx_{j,t}
                       +\alpha_t \nabla f_{i}(\bbx_{i,t}).}$  
          %
   \IF{$\|\bbg_{i,t}\|\leq tol$}
   \STATE Set $s_{ii}=1$.
   \STATE Send scalar $1$ to all nodes.
   \ENDIF
   
   
   \STATE Set $s_{ij}=1$ for all nodes $j$ that sent a signal.

   
   \IF{$s_{ij}=1$ for all $j=1,\dots,n$}
   \STATE Update penalty parameter $\alpha_{t+1}=\alpha_t/10.$
   \STATE Set $s_{ij}=0$ for all $j=1,\dots,n$.
   \ELSE
   \STATE Use the old $\alpha$: $\alpha_{t+1}=\alpha_t.$
   \ENDIF
   
   \STATE Compute NN-0 descent direction $\bbd_{i,t}^{(0)}=-\bbD_{ii,t}^{-1}\ \!\bbg_{i,t}$ 
   \FOR  {$k=  0, \ldots, K-1$ } 
      \STATE Exchange local elements $\bbd_{i,t}^{(k)}$ of the NN-$k$ step with neighbors
      \STATE NN-$(k+1)$ step:
             %
             $\displaystyle{  
             \bbd_{i,t}^{(k+1)} = \bbD_{ii,t}^{-1}\!
             			\left[
                                   \sum_{j\in \mathcal{N}_i,j=i}\!\!\!\!\!\bbB_{ij} \bbd_{t,j}^{(k)} 
                                    - \bbg_{i,t}\right]}$.        
   \ENDFOR
  %  $\bbD_t_{N}(t)=$ NN Descent Direction $\left(\bbD_t_{0}(t), \bbg(t), N \right)$.
          %
          \STATE Update local iterate: 
          $\displaystyle{\bbx_{i,t+1}=\bbx_{i,t} +\eps\ \bbd_{i,t}^{(K)}}$.
\ENDFOR}
\end{algorithmic}\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


As mentioned in Section \ref{sec:problem}, NN-$K$ algorithm instead of solving optimization problem \eqref{original_optimization_problem1} or its equivalent problem \eqref{original_optimization_new_notation}, solves a penalty version of \eqref{original_optimization_new_notation} as introduced in \eqref{centralized_opt_problem}. 
The optimal solution of optimization problem \eqref{original_optimization_new_notation}, $\tby^*=[\bbx^{*};\ldots;\bbx^{*}]$, is different from the optimal solution of optimization problem \eqref{centralized_opt_problem} $\bby^*$ and the gap between $\tby^*$ and $\bby^*$ is upper bounded by $O(\alpha/(1-\rho))$ where $\alpha $ is the penalty parameter and $\rho$ is the second largest eigenvalue modulus of weight matrix $\bbW$ \cite{YuanQing}. This observation implies that by setting a decreasing policy for the penalty parameter $\alpha$, the solution of  \eqref{original_optimization_new_notation} approaches the minimizer of  \eqref{centralized_opt_problem}, i.e. $\tby^* \to \bby^*$ for $\alpha\to  0$.

Different policies for updating the penalty factor can be considered. A simple and trivial  policy is to increase penalty coefficient $1/\alpha_t $ or equivalently decrease $\alpha_t$, e.g. dividing $\alpha_{t+1}=\alpha_t/10$, after completing a specific number of iterations. These jumps in the value of parameter $\alpha_t$ can be optimized empirically. The more accurate way is that each node observes the norm of its local gradient and when it reaches a specific threshold it sends a signal to the other nodes in the network. When all the nodes in the network send the same signal they all decrease $\alpha_t$ or divide it by a specific constant. Using this procedure all the nodes in the network update the parameter $\alpha_t$ simultaneously. Since the number of times that $\alpha_t$ should be updated is small, the cost of communication for updating $\alpha_t$ is affordable. 

We introduce Adaptive Network Newton-$K$ (ANN-$K$) as a version of NN-$K$ that uses a decreasing sequence of $\alpha_t$ to achieve exact convergence to the optimal solution of \eqref{original_optimization_problem1}. The idea of ANN-$K$ is to decrease parameter $\alpha$ when the sequence generated by NN-$K$ is converged for a specific value of $\alpha$. To be more precise, each node $i$ has a \textit{signal vector} $\bbs_{i}=[s_{i1};\dots;s_{in}]\in \{0,1\}^n$ where each component is a binary variable. Each node $i$ at each iteration $t$ computes its local gradient norm $\|\bbg_{i,t}\|$ and if the norm of gradient is smaller than a specific value called $tol$, i.e. $\|\bbg_{i,t}\|\leq tol$, it sets the local signal component to $s_{ii}=1$ and sends the signal to all the nodes in the network. The receiver nodes set the corresponding component of node $i$ in their local signal vectors to 1, i.e. $s_{ji}=1$ for $j\neq i$. This procedure implies that the local signal  vectors $\bbs_{i}$ are always synchronous. The update for parameter $\alpha_t$ occurs when all the components of signal vector are 1 which is equivalent to achieving the required accuracy for all nodes in the network. 

The ANN-$K$ method is summarized in Algorithm \ref{algo_ANN}. The difference between NN-$K$ and ANN-$K$ is in using signal vectors for updating penalty parameter $\alpha$. In Steps 4-7 the local signal component $s_{ii}$ is updated and sent  to the other nodes if the accuracy $\|\bbg_{i,t}\|\leq tol$ is achieved for node $i$. In Step 8 each node $i$ updates the signal vector components of other nodes in the network. Finally, in Steps 9-14 the nodes update the penalty parameter for the next iteration as $\alpha_{t+1}=\alpha_t /10$  if all the components of signal vector is 1, otherwise they keep the same value $\alpha_{t+1}=\alpha_{t}$. In order to reset the system after updating $\alpha_t$ all local signal vectors set to 0, i.e. $\bbs_{i}=\bb0$ for $i=1,\dots,n$.

\begin{remark}
{One may think for achieving more exact convergence instead of using the ANN-$K$ method with decreasing $\alpha $ the NN-$K$ algorithm with very small penalty factor can be used, however, this choosing very small $\alpha$ leads to very slow convergence for NN-$K$. By setting large $\alpha $ we try to minimize objective function $\sum_{i=1}^n f_{i}(\bbx)$ with less concern about the constraint $(\bbI-\bbZ)^{1/2}\bby=\bb0$. This leads to a point closer to the optimal solution. Then, by decreasing $\alpha $ we put more weight on the constraint and less on the objective function, while we use a better initial point than just starting the whole procedure with small $\alpha$. This is well studied in Section \ref{sec:simulations}.}
\end{remark}






